On Reducing Decoding Complexity of Successive-Cancellation List Flip Decoding of Polar Codes

The recently proposed SCLF decoding algorithm for polar codes improves the error-correcting performance of state-of-the-art SCL decoding. However, it comes at the cost of a higher complexity. In this paper, partitioned polar codes tailored for the proposed PSCLF decoding algorithm are used to reduce the complexity of SCLF. Indeed, compared to SCLF, PSCLF allows early termination and is able to restart by skipping part of the decoding tree traversed sequentially. In order to maximize the coding gain, design of partitions tailored to PSCLF is proposed. In this extended paper, dynamic flip metric is used, as well as the possibility to flip multiple times during SCL. An analysis on the impact of this strategy on the early-termination or the CRC collisions encountered in PSCLF is carried out. Error-correction performance of multiple code rates and multiple partition strategies are shown. With the baseline algorithm SCL with $L=2$, degradation of $0.05$ dB is shown with respect to SCL-64, using $\omega=3$ flip per trial with $T_{max}=300$ trials. Numerical results show that the proposed PSCLF algorithm has an error-correction performance gain of up to 0.1 dB with respect to SCLF with same decoding parameters. This work is also compared with existing techniques to reduce the complexity of the SCLF decoding algorithm. The proposed algorithm reduces the complexity up to 77 % at the frame-error rate of $0.01$ with respect to SCLF and is able to reduce more the decoding complexity of SCLF embedding as well a restart mechanism. The average execution time of PSCLF matches the latency of SCL at $\text{FER}=4\cdot10^{-3}$ and lower.

==> 1024_256_mu_P4_w2.tex <==
Eb SNR stddev FERdivK FER
3 -3.0206 1.41589 0.684932 0.549451
3.25 -2.7706 1.37572 0.469484 0.458716
3.5 -2.5206 1.33669 0.334448 0.21322
3.75 -2.2706 1.29876 0.156006 0.107527
4 -2.0206 1.26191 0.0640205 0.0472144
4.25 -1.7706 1.22611 0.0230574 0.013245
4.5 -1.5206 1.19132 0.00778271 0.00473776
4.75 -1.2706 1.15752 0.00213106 0.00165637
5 -1.0206 1.12468 0.000636221 0.000527599
5.25 -0.7706 1.09277 0.000229462 0.000165635
5.5 -0.5206 1.06177 5.86667e-05 NaN


==> 1024_512_diff_crc_avg_exec_time.tex <==
FER8888 avg8888 FER77711 avg77711 FER11777 avg11777
1 250617.84 1 306290.75 1 275819.02
1 257308.97 1 300609.08 1 266142.07
1 285395.61 1 277080.78 1 257963.09
0.990099 281229.0685 1 277537.69 1 275975.61
0.990099 263546.0894 1 277851.82 0.970874 267169.1088
0.952381 249644.9805 0.990099 278781.8038 0.990099 261728.874
0.925926 234640.3641 0.917431 264305.1499 0.925926 230204.4778
0.694444 162188.0194 0.729927 193230.2982 0.680272 157701.8493
0.460829 104564.0488 0.505051 143829.8311 0.434783 103035.0111
0.234742 58333.7423 0.250627 71165.2017 0.178891 41629.67256
0.0664452 19174.80482 0.084246 25548.45409 0.0651042 15908.78618
0.018843 7034.9365 0.0235793 9007.17851 0.0224215 7188.862506
0.00416858 3501.365178 0.00722491 4469.930375 0.00425242 3303.203174
0.000913576 2804.2157968 0.00143017 2965.8213712 0.00106905 2750.8289187
0.000194674 2646.79176348 0.000287172 2687.48038206 0.000265206 2637.98884491
5.2e-05 2619.76179957 5.6e-05 2626.42562847 9.2e-05 2618.59809772
1.06667e-05 2615.445874637 9.33333e-06 2615.677443825 2.8e-05 2614.71141048


==> 1024_512_mu_P4_w2.tex <==
Eb SNR stddev FERmueq FER FERdivK
3 -0.0103 1.00119 1 0.990099 1
3.25 0.2397 0.972781 0.961538 0.980392 0.971
3.5 0.4897 0.945181 0.884956 0.917431 0.926
3.75 0.7397 0.918364 0.628931 0.740741 0.8
4 0.9897 0.892308 0.497512 0.485437 0.568
4.25 1.2397 0.866992 0.241546 0.26455 0.273
4.5 1.4897 0.842393 0.0888889 0.0896057 0.116
4.75 1.7397 0.818493 0.0287439 0.0237417 0.0256
5 1.9897 0.795271 0.00688468 0.00474901 0.00837
5.25 2.2397 0.772707 0.00199291 0.00107825 0.00206
5.5 2.4897 0.750784 0.000476206 0.00020992 0.000414
5.75 2.7397 0.729483 9.73333e-05 5.33333e-05 0.000156


==> 1024_768_mu_P4_w2.tex <==
Eb SNR stddev FERmueq FER FERdivK
4.75 3.50061 0.668297 0.961538 0.900901 0.98 
5 3.75061 0.649336 0.78125 0.757576 0.87
5.25 4.00061 0.630913 0.568182 0.460829 0.633
5.5 4.25061 0.613013 0.254453 0.21322 0.328
5.75 4.50061 0.59562 0.084674 0.0725163 0.0911
6 4.75061 0.578721 0.0236072 0.0169147 0.0269
6.25 5.00061 0.562302 0.00599916 0.00371361 0.00761
6.5 5.25061 0.546348 0.00120084 0.000673002 0.00124
6.75 5.50061 0.530847 0.000418261 0.000136575 0.000391
7 5.75061 0.515786 0.000170352 NaN 0.000145


==> SCL_1024_256.tex <==
Eb SNR stddev SCL2 SCL16
2.25 -3.7706 1.54358 0.995025 0.985222
2.5 -3.5206 1.49979 0.985222 0.892857
2.75 -3.2706 1.45724 0.97561 0.884956
3 -3.0206 1.41589 0.917431 0.655738
3.25 -2.7706 1.37572 0.796813 0.454545
3.5 -2.5206 1.33669 0.647249 0.28777
3.75 -2.2706 1.29876 0.480769 0.148258
4 -2.0206 1.26191 0.316456 0.0580889
4.25 -1.7706 1.22611 0.185874 0.0223839
4.5 -1.5206 1.19132 0.0810373 0.00588737
4.75 -1.2706 1.15752 0.0409082 0.00134113
5 -1.0206 1.12468 0.015348 0.00027826
5.25 -0.7706 1.09277 0.00535375 NaN
5.5 -0.5206 1.06177 0.00177421 NaN
5.75 -0.2706 1.03164 0.000518722 NaN
6 -0.0205999 1.00237 0.000138667 NaN


==> SCL_1024_512.tex <==
Eb SNR stddev SCL2 SCL16 SCL64 lat16 lat64 
3.5 0.4897 0.945181 0.995025 0.858369 0.790514 37990.0096 142503.9296
3.75 0.7397 0.918364 0.938967 0.699301 0.56 34576.1856 114648.0704
4 0.9897 0.892308 0.83682 0.469484 0.3 25179.66784 74812.0768
4.25 1.2397 0.866992 0.647249 0.225734 0.1344 18631.13472 42172.6656
4.5 1.4897 0.842393 0.409836 0.0735024 0.03546 10837.3824 18395.57824
4.75 1.7397 0.818493 0.169205 0.0208117 0.0058184 6083.29792 7781.65568
5 1.9897 0.795271 0.0802246 0.00434339 0.0009823 3646.12672 4042.48192
5.25 2.2397 0.772707 0.030248 0.000698156 0.0001033 2666.74496 2714.42304
5.5 2.4897 0.750784 0.00765873 8.53333e-05 5.33e-06 2279.382208 2282.042944
5.75 2.7397 0.729483 0.00203791 6.66667e-06 NaN 2141.22336 NaN
6 2.9897 0.708786 0.000484885 NaN NaN NaN NaN
6.25 3.2397 0.688676 0.0001146 NaN NaN NaN NaN

==> SCL_1024_768.tex <==
Eb SNR stddev SCL2 SCL16
4.75 3.50061 0.668297 0.995025 0.97561
5 3.75061 0.649336 0.947867 0.760456
5.25 4.00061 0.630913 0.858369 0.543478
5.5 4.25061 0.613013 0.619195 0.27137
5.75 4.50061 0.59562 0.367647 0.0825083
6 4.75061 0.578721 0.166528 0.0177541
6.25 5.00061 0.562302 0.0616713 0.00284047
6.5 5.25061 0.546348 0.0167476 0.000334407
6.75 5.50061 0.530847 0.00460278 4.4e-05
7 5.75061 0.515786 0.00117943 8e-06
7.25 6.00061 0.501152 0.000314247 NaN

